Importance Estimation for Neural Network Pruning

Structural pruning of neural network parameters reduces computation, energy, and memory transfer costs during inference. We propose a novel method that estimates the contribution of a neuron (filter) to the final loss and iteratively removes those with smaller scores. We describe two variations of our method using the first and second-order Taylor expansions to approximate a filter's contribution. Both methods scale consistently across any network layer without requiring per-layer sensitivity analysis and can be applied to any kind of layer, including skip connections. For modern networks trained on ImageNet, we measured experimentally a high (>93%) correlation between the contribution computed by our methods and a reliable estimate of the true importance. Pruning with the proposed methods leads to an improvement over state-of-the-art in terms of accuracy, FLOPs, and parameter reduction. On ResNet-101, we achieve a 40% FLOPS reduction by removing 30% of the parameters, with a loss of 0.02% in the top-1 accuracy on ImageNet. Code is available at https://github.com/NVlabs/Taylor_pruning.

==> tables/table_resnet50_cor.tex <==
\begin{table}
\centering
%\scriptsize
\resizebox{\linewidth}{!} %\linewidth
{
\begin{tabular}{lcccc}
\toprule
Method & \multicolumn{2}{c}{Averaged per layer} &  \multicolumn{2}{c}{Over all layers} \\ 
 & Spearman & Kendall  & Spearman$\downarrow$ & Kendall \\

\midrule
Taylor FO on gate  & \textbf{.9669} & \textbf{.8727}      & \textbf{.9725}   & \textbf{.8824} \\
% Hybrid &  .9648 &  .8647    & .9677   &  .8488 \\
Taylor FO on gate - full grad & .9307 & .7969  & .9632 & .8422   \\ 
Taylor FO on conv weight& .9386& .8063  & .9431 & .8057 \\
Taylor SO on gate   & .9625 & .8593     & .9403   & .8040 \\
Weight magnitude    &  .8972   &  .7470      &  .9164    & .7561 \\
ICLR2017 \cite{ICLR2017}  & .8935 & .7408     & .8912   & .7248 \\
OBD on gate         & .8281 & .6815      & .7457   & .5621 \\
\bottomrule
\end{tabular}
}
\caption{Correlation study of different criteria and oracle on CIFAR10 with ResNet50. Computed for randomly selected 1280 images. The exact importance of neuron was computed by setting every convolutional filter to zero and estimating resulting quadratic change in loss.}
\label{tab:resnet50_corr}
\end{table}


==> tables/table_yolo_results.tex <==
\begin{table}
\centering
%\scriptsize
\resizebox{0.95\linewidth}{!}
{
\begin{tabular}{lccccc}
\toprule
Pruning Method & GFLOPs & Params($10^7$) & Precision & Recall & F1 score\\ 
\midrule
No pruning  & 14.68 & 5.07 & .712 & .728 & .717\\
{Taylor-FO-BN-70\% (Ours)}  & 9.15 & 1.98 & .707 & .726 & .714\\
{Taylor-FO-BN-50\% (Ours)}  & 6.76 & 1.03 & .683 & .728 & .702\\

\bottomrule
\end{tabular}
}
\caption{Pruning results on YOLOv2 on Pascal VOC 2007.}
\label{tab:yolo_acc}
% \vspace{-10pt}
\end{table}

